Observation and measurements of the production of prompt and non-prompt $J/\psi$ mesons in association with a $Z$ boson in $pp$ collisions at $\sqrt{s}= 8$ TeV with the ATLAS detector

The production of a $Z$ boson in association with a $J/\psi$ meson in proton-proton collisions probes the production mechanisms of quarkonium and heavy flavour in association with vector bosons, and allows studies of multiple parton scattering. Using $20.3\, \mathrm{fb^{-1}}$ of data collected with the ATLAS experiment at the LHC in $pp$ collisions at $\sqrt{s}=8\, \mathrm{TeV}$, the first measurement of associated $Z + J/\psi$ production is presented for both prompt and non-prompt $J/\psi$ production, with both signatures having a significance in excess of $5\sigma$. The inclusive production cross-sections for $Z$ boson production (analysed in $\mu^+\mu^-$ or $e^+e^-$ decay modes) in association with prompt and non-prompt $J/\psi(\to\mu^+\mu^-)$ are measured relative to the inclusive production rate of $Z$ bosons in the same fiducial volume to be $(36.8\pm 6.7\pm 2.5) \times 10^{-7}$ and $(65.8\pm 9.2\pm 4.2) \times 10^{-7}$ respectively. Normalised differential production cross-section ratios are also determined as a function of the $J/\psi$ transverse momentum. The fraction of signal events arising from single and double parton scattering is estimated, and a lower limit of $5.3\ (3.7)\, \mathrm{mb}$ at $68\ (95)$% confidence level is placed on the effective cross-section regulating double parton interactions.

==> mycommands.tex <==
%%%%%%%%%%%%%
%%% Re-Define name for Table Of Contents (default is "Contents")
%\renewcommand{\contentsname}{Table of Contents}

%\def \integrated{$ 3.04 \pm  0.93 \textrm{(stat)} ^{+ 0.18 }_{- 0.12 }\textrm{(syst)} $ }
\def \signalyield{$27.4^{+7.5} _{-6.5} $}
\def \origsignalyield{$29.2^{+7.5} _{-6.5} $}
%\def \significance{$5.3\sigma$}
\def \significance{$5.1\sigma$}
\def \MET {\ensuremath{\slashed{E}_{T}}\xspace} %{E^{miss}_{T}}
\def \ME {$\slashed{E}$\xspace}
\def \wenu {$W \to e \nu$\xspace}
\def \wmunu {$W \to \mu \nu$\xspace}
\def \zee {$Z \to ee$\xspace}
\def \zmumu {$Z \to \mu^+ \mu^-$\xspace}
\def \jets {\mathrm jets}
\def \jpsi {\ensuremath{\Jpsi}\xspace}
\def \Zboson {\ensuremath{Z}\xspace}
\def \w {\ensuremath{W}\xspace}
\def \Zbosonjpsi {$\Zboson + \Jpsi$\xspace}
\def \Zbosonjpsi {$\Zboson + \textrm{prompt} ~\Jpsi$\xspace}
\def \ifb {fb$^{-1}$\xspace}
\def \ratio {\ensuremath{R_{\jpsi}}\xspace}
\newcommand{\ratiofull}{\ensuremath{\mathrm{BR}(\jpsi\rightarrow\mu\mu)(1/\sigma_\mathrm{fid}(pp \to \Wpm)) d^{2}\sigma_\mathrm{fid}(pp \to \Wpm + \Jpsi) / dy\ dp_{T}}\xspace}
\def \WTM {\ensuremath{m_\textrm{T}(\w)}\xspace}
\def \QCD {QCD\xspace}
\def \NRQCD {NRQCD\xspace}
\def \MC {MC\xspace}
\def \GeV {GeV\xspace}
\def \PDF {PDF\xspace}
\def \LHC {LHC\xspace}
\def \ATLAS {ATLAS\xspace}
\newcommand{\ptjpsi}{\ensuremath{\pt^{\jpsi}}\xspace}
\newcommand{\yjpsi}{\ensuremath{y_{\jpsi}}\xspace}
\newcommand{\lumimeanmu}{\ensuremath{\langle\mu\rangle}\xspace}
\newcommand{\rfid}{\ensuremath{R_{\jpsi}^\mathrm{fid}}\xspace}
\newcommand{\rincl}{\ensuremath{R_{\jpsi}^\mathrm{incl}}\xspace}
\newcommand{\rdpssub}{\ensuremath{R_{\jpsi}^\textrm{DPS sub}}\xspace}


==> zjpsiCOVER.tex <==
%-------------------------------------------------------------------------------
% This file contains the title, author and abstract.
% It also contains all relevant document numbers used by the different cover pages.
%-------------------------------------------------------------------------------

%% Title
\AtlasTitle{Observation and measurements of the production of prompt and non-prompt {\boldmath $\Jpsi$} mesons in association with a {\boldmath $Z$} boson in {\boldmath $pp$} collisions at {\boldmath $\sqrt{s}= 8\,\mathrm{TeV}$} with the ATLAS detector}

%
% Author - this does not work with revtex
% \author{The ATLAS Collaboration}
%
% Date: if not given, uses current date
% \date{\today}

% Draft version:
% Should be 1.0 for the first circulation, and 2.0 for the second circulation.
% If given, adds draft version on front page, a 'DRAFT' box on top of each other page, 
% and line numbers.
% Comment or remove in final version.
\AtlasVersion{2.0}

% ATLAS reference code, to help ATLAS members to locate the paper
\AtlasRefCode{BPHY-2014-01}

% ATLAS note number. Can be an COM, INT, PUB or CONF note
\AtlasNote{ATLAS-COM-PHYS-2014-412}	 

% Submission journal
\AtlasJournal{EPJC}

% Abstract - % directly after { is important for correct indentation
\AtlasAbstract{
The production of a $Z$ boson in association with a $J/\psi$ meson in proton--proton collisions probes the production mechanisms of quarkonium and heavy flavour in association with vector bosons, and allows studies of multiple parton scattering. Using $20.3\,\mathrm{fb^{-1}}$ of data collected with the ATLAS experiment at the LHC, in $pp$ collisions at $\sqrt{s}=8\,\mathrm{TeV}$, the first measurement of associated $Z\, +\, J/\psi$ production is presented for both prompt and non-prompt $J/\psi$ production, with both signatures having a significance in excess of $5\sigma$. The inclusive production cross-sections for $Z$ boson production (in $\mu^+\mu^-$ or $e^+e^-$ decay modes) in association with prompt and non-prompt $J/\psi(\to\mu^+\mu^-)$ are measured relative to the inclusive production rate of $Z$ bosons in the same fiducial volume to be $(88\pm 16\pm 6)\, \times\, 10^{-8}$ and $(157\pm 22\pm 10)\, \times\, 10^{-8}$ respectively. Normalised differential production cross-sections are also determined as a function of the \Jpsi\ transverse momentum. The fraction of signal events arising from single and double parton scattering is estimated, and a lower limit of $5.3\ (3.7)\,\mathrm{mb}$ at $68\ (95) \%$ confidence level is placed on the effective cross-section regulating double parton interactions.

% \DocumentStyle.
}

%-------------------------------------------------------------------------------
% The following information is needed for the cover page. The commands are only defined
% if you use the coverpage option in atlasdoc or use the atlascover package
%-------------------------------------------------------------------------------

% Explicit list of supporting notes  (leave as null \AtlasCoverSupportingNote{} if you want to skip this option)
\AtlasCoverSupportingNote{A supporting note}{http://cds.cern.ch/record/1699862}
%
% OR (the 2nd option is deprecated, especially for CONF and PUB notes)
%
% Supporting material TWiki page  (leave as null \AtlasCoverTwikiURL{} if you want to skip this option)
% \AtlasCoverTwikiURL{https://twiki.cern.ch/twiki/bin/view/Atlas/WebHome}

% Comment deadline
\AtlasCoverCommentsDeadline{12 November 2014}

% Analysis team members -- Indicate the Contact Editors (usually two) by (*) after their name
\AtlasCoverAnalysisTeam{Theodoros Alexopoulos, James Catmore(*), Vato Kartvelishvili, Stefanos Leontsinis(*), Darren Price, Miriam Watson(*)}

% Editorial Board Members --- Indicate the Chair by a (*) after his/her name
\AtlasCoverEdBoardMember{Sandro Palestini(*), Soeren Prell, Joost Vossebeld, Zhiqing Zhang}

% Editors egroup
\AtlasCoverEgroupEditors{atlas-bphy-2014-01-editors@cern.ch}

% EdBoard egroup
\AtlasCoverEgroupEdBoard{atlas-bphy-2014-01-editorial-board@cern.ch}

% CERN preprintnumber
\PreprintIdNumber{CERN-PH-2014-XX}

